Modeling the meteoroid environment far from the ecliptic plane

We describe a new version (numbered 3.1) of NASA's Meteoroid Engineering Model (MEM) in which we extend the model to handle locations that lie more than a few degrees in latitude off the ecliptic plane. We provide our algorithms for computing the spatial density and directionality of meteoroids far from the ecliptic and discuss their applications. In particular, we demonstrate how correct modeling of the out-of-ecliptic environment is critical for accurately assessing the risk posed by meteoroids to solar observation missions such as Solaris.

==> abstract.tex <==
We describe a new version (numbered 3.1) of NASA's Meteoroid Engineering Model (MEM) in which we extend the model to handle locations that lie more than a few degrees in latitude off the ecliptic plane. We provide our algorithms for computing the spatial density and directionality of meteoroids far from the ecliptic and discuss their applications. In particular, we demonstrate how correct modeling of the out-of-ecliptic environment is critical for accurately assessing the risk posed by meteoroids to solar observation missions such as \emph{Solaris}.

